Not All Diffusion Model Activations Have Been Evaluated as Discriminative Features

Diffusion models are initially designed for image generation. Recent research shows that the internal signals within their backbones, named activations, can also serve as dense features for various discriminative tasks such as semantic segmentation. Given numerous activations, selecting a small yet effective subset poses a fundamental problem. To this end, the early study of this field performs a large-scale quantitative comparison of the discriminative ability of the activations. However, we find that many potential activations have not been evaluated, such as the queries and keys used to compute attention scores. Moreover, recent advancements in diffusion architectures bring many new activations, such as those within embedded ViT modules. Both combined, activation selection remains unresolved but overlooked. To tackle this issue, this paper takes a further step with a much broader range of activations evaluated. Considering the significant increase in activations, a full-scale quantitative comparison is no longer operational. Instead, we seek to understand the properties of these activations, such that the activations that are clearly inferior can be filtered out in advance via simple qualitative evaluation. After careful analysis, we discover three properties universal among diffusion models, enabling this study to go beyond specific models. On top of this, we present effective feature selection solutions for several popular diffusion models. Finally, the experiments across multiple discriminative tasks validate the superiority of our method over the SOTA competitors. Our code is available at https://github.com/Darkbblue/generic-diffusion-feature.

==> secs/mech_fig.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=.52\linewidth]{pics/mech-granularity.jpg}
  \includegraphics[width=.45\linewidth]{pics/mech-multi-vit.jpg}
  \caption{Granularity Rule: The granularity spectrum of SDXL U-Net spans in three denser and denser tiers, including the sparse spectrum of resolution levels, the moderate spectrum within one level, and the dense spectrum in cooperating ViTs.}
  \label{fig:mech-granularity}
\end{figure*}

==> secs/method_fig.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{pics/method.jpg}
  \caption{We propose a feature extraction principle based on the three important rules of U-Net behaviors, each corresponding to a decision consisting the principle (a,b,c).
  Practical solutions can be made according to the principle for various diffusion models, here exemplified by SDXL.}
  \label{fig:method}
\end{figure*}
